Automated Predicate Abstraction for Real-Time Models

We present a technique designed to automatically compute predicate abstractions for dense real-timed models represented as networks of timed automata. We use the CIPM algorithm in our previous work which computes new invariants for timed automata control locations and prunes the model, to compute a predicate abstraction of the model. We do so by taking information regarding control locations and their newly computed invariants into account.

==> eptcsdata.tex <==
\providecommand{\event}{Axel Legay and Azadeh Farzan (Eds.): International Workshop on Verification of Infinite-State Systems (INFINITY 2009)}
\providecommand{\volume}{10}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{36}
\providecommand{\eid}{3}

